NAIL: Lexical Retrieval Indices with Efficient Non-Autoregressive Decoders

Neural document rerankers are extremely effective in terms of accuracy. However, the best models require dedicated hardware for serving, which is costly and often not feasible. To avoid this serving-time requirement, we present a method of capturing up to 86% of the gains of a Transformer cross-attention model with a lexicalized scoring function that only requires 10-6% of the Transformer's FLOPs per document and can be served using commodity CPUs. When combined with a BM25 retriever, this approach matches the quality of a state-of-the art dual encoder retriever, that still requires an accelerator for query encoding. We introduce NAIL (Non-Autoregressive Indexing with Language models) as a model architecture that is compatible with recent encoder-decoder and decoder-only large language models, such as T5, GPT-3 and PaLM. This model architecture can leverage existing pre-trained checkpoints and can be fine-tuned for efficiently constructing document representations that do not require neural processing of queries.

==> model.tex <==
\section{Document Indexing Model with Non-Autoregressive Decoder}
\label{sec:model}

In this section we describe the construction of a model used for indexing documents for retrieval, by precomputing a distribution of scores over the model vocabulary ($\mathcal{MV}$).

\subsection{Non-Autoregressive Decoder}

Non-autoregressive sequence-to-sequence models have been previously proposed and studied, particularly in the context of machine translation~\cite{nonautoregressive-translation,parallel-wavenet,deterministic-nonautoregressive}. These, and other related models, have been motivated by the computational complexity of standard auto-regressive decoding, which requires a decode step per generated token. Non-autoregressive decoding breaks the inter-step dependency and thus provides two computational benefits: (1) a single step through the decoder can produce outputs for more than one position, (2) computation can be easily parallelized since there is no time-wise dependencies between computations.

Specifically, we can model the probability of a query ($q$) given a document ($d$) with the model:
\[
p(\mathbf{q} | \mathbf{d}) = \prod_{t=1}^{n}{p(q_{t} | \mathbf{d} ; \theta} )
\]
where $\theta$ is the set of model parameters. In this model, each token of the query $q$ ($q_{t}$) is modelled conditionally only on the input document $d$. This allows output distributions to be computed in parallel at inference time.

In terms of model architecture, we aim to adapt the decoder architecture of existing large language models, typically trained in auto-regressive fashion, and introduce non-autoregressive decoding for training and inference.


TLDR: We take a standard encoder-decoder or prefix-lm models, modifying it to produce one-shot parallel non-autoregressive decodes. This involves three modifications:
\begin{enumerate}
    \item Modify inputs to the decoder: during training, no teacher forcing of gold inputs, but rather a unique, trained, embedding for all positions. During inference, we do not iterate, but take the output after the first step.
    \item Take the outputs of each position and pool them to produce a single representation.
    \item (Optional) Decoder attention can be modified so that, instead of enforcing a causal attention pattern from the original auto-regressive decoder, a bi-directional attention pattern is allowed. This change in attention pattern proved to be unecessary.
\end{enumerate}

Figure~\ref{fig:model-architecture} illustrates the non-autoregressive decoder.

TODO: Talk about motivation and advantages behind not using a (more powerful) auto-regressive decoder.

\subsection{Generative and Contrastive Losses}

Specifically, we model the interaction between a document weight vector, $\mathbf{w_{d}}$, and a query weight vector $\mathbf{w_{q}}$. Consistent with the constraints described in Section~\ref{sec:task}, the query weight vector is constructed by simply tokenizing the query $q$ into $[t_0, ..., t_n]$ terms and assigning of weight of 1 to each term:
\[
\mathbf{w_{q}} = \sum_{t \in q}{onehot(t)}
\]
Where $onehot(i)$ corresponds to the unary vector with $i$-th position set to 1 and all other positions set to 0.

The weight vector $\mathbf{w_{d}}$ is determined by a learned model $f_{\theta}(d)$.

Given a set of positive training examples $\{(d_{0}, q_{0}) ... (d_{n}, q_{n})\}$ we seed to learn $f_{\theta}(d)$ such that the inner product
$\langle \mathbf{w_{d_{i}}} \cdot \mathbf{w_{q_{j}}} \rangle$ is maximal when $i = j$. This is equivalent to maximizing the sum of document term weights that appear in the query:
\[
s(q_j, d_i) = \sum_{t \in q}{\mathbf{w_{d_{i}}}^{t}}
\]


\subsubsection{Generative-based loss}

\subsubsection{Contrastive-based loss}



==> task.tex <==
\section{Task Definition: Fast Retrieval using Precomputed Term Scores}
\label{sec:task}


The goal of a retrieval system is to, given a query $q$, return an ordered list of documents $d_{1}, d_{2}, ..., d{n}$ from a retrieval corpus $\mathcal{C}$. In this work, we focus on query scoring functions that use lexical or token-based inverted indices so that interactions between query terms and documents are \emph{precomputed} and stored in an efficiently accessible data-structure. Specifically, the family of scoring functions we consider are:
\begin{equation}
  s(q, d) = \mathcal{F}_{qd} (\mathcal{F}_{q}(q, \mathcal{RV}), \mathcal{F}_{d}(d, \mathcal{RV}))
\end{equation}
where $\mathcal{RV}$ is the set of all terms in a precomputed retrieval vocabulary, typically determined at document indexing time. $\mathcal{F}_{d}(d, \mathcal{V})$ is a function that, given a document $d \in \mathcal{C}$ produces a score for each term in $\mathcal{RV}$, and similarly, $\mathcal{F}_{q}(q, \mathcal{V})$ is a function that, given a query $q$ produces a score for each term in $\mathcal{RV}$. In this work we focus on variants of $\mathcal{F}_{d}$ that may be computationally expensive (since costs of index construction can be amortized over time) and classes of $\mathcal{F}_{q}$ that are trivial to compute, involving no neural network (e.g., tokenization).

Note that the BM25~\cite{bm25}, and other variants of TF-IDF based retrieval systems are examples of the above task formulation.

Most of the work presented in this paper focuses a simplification of the above score function by considering $\mathcal{RV}$ vocabularies that correspond to unigram terms of model vocabulary ($\mathcal{MV}$) used in a large language model. We show that this simplification allows us to construct efficient models for document indexing compared to vocabularies that require sequences of individual terms.


